Who watches the watchers: Validating the ProB Validation Tool

Over the years, ProB has moved from a tool that complemented proving, to a development environment that is now sometimes used instead of proving for applications, such as exhaustive model checking or data validation. This has led to much more stringent requirements on the integrity of ProB. In this paper we present a summary of our validation efforts for ProB, in particular within the context of the norm EN 50128 and safety critical applications in the railway domain.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{Dubois C., Giannakopoulou D., Méry D. (Eds): Formal Integrated\\Development Environment 2014 (F-IDE 2014)\\
EPTCS 149, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.149.3}{10.4204/EPTCS.149.3}}
\pdfoutput=1

